DAPES: Named Data for Off-the-Grid File Sharing with Peer-to-Peer Interactions

This paper introduces DAta-centric Peer-to-peer filE Sharing (DAPES), a data sharing protocol for scenarios with intermittent connectivity and user mobility. DAPES provides a set of semantically meaningful hierarchical naming abstractions that facilitate the exchange of file collections via local connectivity. This enables peers to "make the most" out of the limited connection time with other peers by maximizing the utility of individual transmissions to provide data missing by most connected peers. DAPES runs on top of Named-Data Networking (NDN) and extends NDN's data-centric network layer abstractions to achieve communication over multiple wireless hops through an adaptive hop-by-hop forwarding/suppression mechanism. We have evaluated DAPES through real-world experiments in an outdoor campus setting and extensive simulations. Our results demonstrate that DAPES achieves 50-71% lower overheads and 15-33% lower file sharing delays compared to file sharing solutions that rely on IP-based mobile ad-hoc routing.

==> 4-analysis.tex <==
\section{Analytical Modeling}
\label{sec:analysis}

In this section, we present some analysis of our design. 

%Time delay and transmission overhead are two important metrics for evaluating the proposed nTorrent data sharing protocol design. In this section we first analyze the bitmap transmission prioritzation , then ...  

%The work of xxx showed that sth in xx is xxx /ref 

%\subsection{First Time Data Fetching}

%We adopt an algorithm for selecting a randomized starting point when fetching data for the first time. Then a node fetches in sequence for a certain number of data pieces, and repeat the process by selecting another random starting point.

%We meaure the average difference in data pieces carried by encountered nodes in terms of percentage. 

%We also analyze the base case where nodes start by fetching the first data piece of a torrent file. 
%T\textsubscript{data fetching} = t - (T\textsubscript{delay} + d) * b

\subsection {Torrent-File Size}

Following the format of Figure~\ref{Figure:torrent-file1}, the bytes needed to encode the subnames in the content of a torrent-file are: $B\textsubscript{subnames} = N\textsubscript{subnames} * (sizeof(int) + sizeof(digest) + sizeof(TLV format))$, where $N\textsubscript{subnames}$ refers to the number of subnames in the torrent-file, $sizeof(int)$ is the size of each individual packet number, $sizeof(digest)$ is the size of the digest, and $sizeof(TLV format)$ is the size of the type and length fields of each subname TLV\footnote{NDN follows a TLV encoding format~\cite{ndn-packet-format}. The exact size of the type and length fields depends on the type assignment and the size of the value field.}. Let us assume that the size of the torrent is 1MB and the size of each data packet content is 1KB. In this case, the torrent-file will contain 1000 subnames. Let us also assume that the size of an integer is 4 bytes, the digest is a SHA1 hash (20 bytes) and the size of the type and length fields is 8 bytes. Therefore, the size of the subnames is 32KB. Depending on the size of the name of each file in the torrent, the torrent-file will be segmented into, at least, 32 data packets. 

Following the format of Figure~\ref{Figure:torrent-file2} and assuming the use of the efficient Tiger hash~\cite{anderson1996tiger}, the size of the Merkle tree root hash will be 24 bytes. Even if each file in the torrent has a separate Merkle tree, the torrent-file can still fit into a single packet. Note that this format makes the size of the torrent-file independent of the torrent size; the torrent-file size roughly depends on the number and size of each root hash, and the size of each file name in the torrent.

\subsection{Bitmap Transmission Prioritization}
\label{subsec:prioritization}

%Exponential Backoff:

%Our work adopts exponential back off timer for collision avoidance and prioritizing Bitmap retransmissions. After collision happens, the maximum backoff timer is becomes 2c-1 slots, where c is the number of collisions. Nodes are divided into n groups based on their priority level. A peer within group m selects a random delay timer from the range $(2^c-1)(m-1)/n$ to $(2^c-1)m/n$ slot times inclusive. As the number of collisions increase, the delay timer range for each group will increase exponentially, thus lowering the collision rate within each group. 

%Let the total amount of time delay be t, the number of peers be n, the probability they fall in the same group is p, slot time s, thus collision probability $c=2(2^c-1)np/ns$ (assuming transmission delay is 2ms and s is in ms). Then total transmission time $t=2(2^c-1)^2p/s$.

Let us assume that there are $L$ transmission slots in total and nodes are divided into $k$ priority groups, thus there are $n = \floor{\frac{L}{k}}$ slots per group. The nodes in the $jth$ priority group select a random slot s, where $j*n \leq s < (j+1)*n$. Zhu et al~\cite{zhu2011performance} proved that the average number of backoffs before a successful transmission is $N\textsubscript{backoff} = \sum_{i=1}^{\infty} iP\textsubscript{i}$, where $P\textsubscript{i}$ is the probability that a node has collided $i$ times before a successful transmission. The average delay for a peer to successfully transmit its bitmap is $T\textsubscript{delay} = \frac{L\textsubscript{average} - 1}{2} \tau$, where $L\textsubscript{average} = \frac{n - 1}{2}$ is the average contention window size of each peer and $\tau$ the time slot duration.

\subsection{Data Advertisements \& Data Fetching}
\label{data-ad-analysis}

Let us assume that a peer is connected with others for a time interval $t$ and the transmission delay is $d$. Peers can either exchange their bitmaps first and then start data fetching or interleave bitmap exchanges and data fetching. For the former approach, if peers exchange $b$ bitmaps before they start fetching data, the average time interval they will have for data fetching will be:

\begin {equation}
     T\textsubscript{data fetching} =
\begin{cases}
    t - (T\textsubscript{delay} + d) * b,& \text{if }(T\textsubscript{delay} + d) * b < t \\
    0,              & \text{if } (T\textsubscript{delay} + d) * b\geq t
\end{cases}
\label{eq1}
\end {equation}

\noindent where T\textsubscript{delay} is the average delay for a peer to successfully transmit a bitmap, as we explained in Section~\ref{subsec:prioritization}. Equation~\ref{eq1} shows that peers will have time for data fetching only if their overall encounter lasts more than the time they need for the bitmap exchanges.

When peers interleave their bitmap and data fetching exchanges, we assume that after they fetch the first bitmap, they have a equal chance of sending a bitmap Interest or an Interest for torrent data until $b$ bitmaps are exchanged. The average time interval that peers will have for data fetching in this case will be: 

\begin {equation}
     T\textsubscript{data fetching} =
\begin{cases}
    t - (T\textsubscript{delay} + d) * b,& \text{if }T\textsubscript{delay} + d < t \\
    0,              & \text{if } T\textsubscript{delay} + d \geq t
\end{cases}
\label{eq2}
\end {equation}

Based on equation~\ref{eq2}, peers will not have time for data fetching only in the case of very small connections (i.e., they do not have enough time to make a single bitmap exchange).

%the number of data fetched would be $n=(t-bd)/2d (n>=0)$, if we assume peers keep fetching data before connection breaks, n depends on connection time t and total bitmap number b. In case $t \textless bd$, peers don't have the chance to fetch any data. 

%If we interleave the bitmap exchange and data fetching process, we could avoid the case of peers not being able to fetch anything if the connection is short, and provide nodes with the same probability of sending Interest for Data as for sending Bitmap Interest. If we assume each one takes up fifty percent of the total transmission, then the total number of data fetched would be n=t/4d which solely depends on time t.

\subsection{Rarest Piece First Strategy}

Qiu et al~\cite{qiu2004modeling} proved that the effectiveness of file sharing $\eta$ based on the rarest piece first strategy is equal to $\eta \approx 1 - (\frac{\log N}{N})^k$, where $N$ is the number of torrent data packets and $k$ is the number of connected peers sharing data. Assuming that the size of each torrent data packet is 1KB, a torrent of size 5MB will consist of 5,000 packets. Even if $k = 1$, i.e., when a peer has only one other peer within its communication range (e.g., for very short WiFi ranges), $\eta$ will be very close to 1. In the general case, multiple peers might be within the communication range of each other, thus $k > 1$, which slowly increases the efficiency of the rarest piece first strategy and file sharing performance. When $k=0$, peers are isolated from each other, thus $\eta = 0$.

%We adopted two type of data fetching RPF strategies, encounter based RPF and one hop neighbor RPF. For enounter based RPF, 

%What to measure here?

%total number of transmissions. 

%Number of bitmaps kept is b, calculate the number of common missing data, 

==> 6-discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\subsection {Pure Forwarding Nodes}
\label{pure-forwarding}

Peers may meet nodes that do not understand the semantics of DAPES, which we call ``pure forwarding nodes'' (e.g., survivors that have not installed the application on their device). These nodes understand the NDN network layer semantics. Given the broadcast nature of the wireless medium, pure forwarding nodes can store and carry overheard torrent data in their CS, thus satisfying future requests for cached data. They can also opportunistically forward received Interests for torrent data based on a self-learning approach~\cite{shi2017broadcast}. Specifically, after forwarding Interests that bring data back, pure forwarding nodes continue to forward future Interests for the same data. When forwarded Interests do not bring data back, pure forwarding nodes start a suppression timer for the specific data names, ignoring future requests for the same data until the timer expires.

\subsection {Multiple Torrent Sharing}

As discussed in Section~\ref{subsec:peerdisc}, peers that have data for multiple torrents can include the name of each torrent-file in the content of a beacon data packet. In such cases, the communicating peers can exchange data advertisements for more than one torrents, thus downloading multiple torrents in parallel. When peers receive requests for torrent data they do not have, they can follow the self-learning approach mentioned in Section~\ref{pure-forwarding} to opportunistically forward them.

==> Makefile <==
PAPER=ad-hoc-ntorrent
PRJ=ad-hoc-ntorrent

all:
	pdflatex $(PAPER).tex
	bibtex $(PAPER)
	pdflatex $(PAPER).tex
	pdflatex $(PAPER).tex

# Small cheat to allow synchronization between PDF and .tex for supported editors (run `make S=1`)
ifdef S
EXTRA = -synctex=1
endif

${PRJ}.pdf : *.tex *.bib
	pdflatex ${EXTRA} ${PRJ} && \
		(ls ${PRJ}.aux | xargs -n 1 bibtex) && \
		pdflatex ${EXTRA} ${PRJ} && pdflatex ${EXTRA} ${PRJ}

view : ${PRJ}.pdf
	open ${PRJ}.pdf &

.PHONY: clean
clean:
	rm -f *.aux *.log *.blg *.dvi *.bbl

pdf: all


==> discussion.tex <==
There may be cases that multiple peers meet, for example, when A moves into the communication range of B, C and D. Given the ephemeral nature of their encounters, peers can select to fetch the bitmap of only some or all the other peers within their communication range. Peers may also select to first retrieve the selected number of bitmaps and then start downloading torrent data or interleave bitmap and data exchanges. These decisions involve a trade-off between the number of bitmaps peers will retrieve (indicating the knowledge they will have about the available data, or in other words, how efficient their downloading process will be) and how much time they will have to download data. We evaluate the effect of these decisions in Section~\ref{subsec:bitmapeval}. 


The first time peers encounter others, they have 2 alternatives on how to start downloading the torrent: (i) start from the same torrent packet and sequentially download as many packets as possible, or (ii) start from a random packet and download sequential packet blocks. Following the former approach, peers may end up having a very similar set of packets during future encounters. With the latter approach, peers will have different blocks of torrent data, thus disseminating diverse content that other peers may not have. We evaluate the effect of these alternatives in Section~\ref{subsec:data-fetching}.

==> related-work.tex <==
\section {Related Work}
\label{sec:related-work}

Data sharing in off-the-grid scenarios has been an active research area. Previous work in MANET~\cite{rajagopalan2006cross, krifa2009bithoc, sbai2008bithoc, pucha2004ekta, gaddam2009study}, running on top of the IP-based architecture, has relied on routing~\cite{he2002destination, johnson2001dsr, perkins2003ad} for communication across multiple hops. Mobility introduces additional challenges, since established paths break and new ones have to be established. Previous work~\cite{nandan2005co, lee2006code, klemm2003special} has advocated that alternative solutions for multi-hop communication need to be explored (e.g., application-layer gossiping, network coding, link-layer flooding). Security is not considered in the routing and the data sharing process~\cite{yang2004security}, while IP address configuration in such infrastructure-free environments is a challenge on its own~\cite{nesargi2002manetconf, mcauley2000self, misra2001autoconfiguration}.

Our work builds on previous work on peer-to-peer data sharing in NDN. nTorrent~\cite{mastorakis2017ntorrent} is the closest work related to DAPES, but focuses on file sharing over infrastructure networks. ``FileSync/NDN''~\cite{lindblom2013filesync} implemented a peer-to-peer file synchronization in a shared directory among peers, while Detti et al~\cite{detti2013peer, detti2015mobile} and Malabocchia et al~\cite{malabocchia2015using} studied the design of peer-to-peer video streaming applications. 

Previous work has also studied the design of general purpose architectures for MANET in NDN. E-CHANET~\cite{amadeo2013chanet} is such an architecture for MANET that runs on top of IEEE 802.11 and focuses on providing stable paths and reliable transport functions toward named data. Varvello et al.~\cite{varvello2011design} performed an analytical study of various design choices for resource discovery and forwarding in NDN-based MANETs. Meisel et al.~\cite{meisel2010listen} proposed a design for multi-hop MANET forwarding in NDN. In this design, called ``Listen First, Broadcast Later'' (LFBL), nodes learn about the available data around them by overhearing the transmissions broadcasted by others.

DAPES differs from the efforts above. It tackles the problem of data sharing in off-the-grid scenarios through semantically meaningful naming semantics understood by both applications and the NDN network. The NDN stateful forwarding plane and the naming semantics enable DAPES peers to identify what data is available across multiple hops over time, thus achieving multi-hop communication without the need of a ``traditional'' MANET routing protocol. Our multi-hop communication design was inspired by LFBL, however, DAPES extends LFBL's principles to fully utilize the potential understanding of intermediate nodes about the DAPES operations. Furthermore, the cryptographic primitives built into NDN provide a solid foundation for securing the data sharing process.

%\subsection{Peer-to-Peer Data Sharing in IP}

%One of the first designs to study the problem of content sharing in MANETs is SPAWN~\cite{nandan2005co}. SPAWN assumes the existence of moving cars and stationary gateways; a car connects to a gateway to download torrent pieces, and receive a list of cars interested in the same torrent that were recently connected to the same gateway. Once a car gets out of the gateway range, it continues downloading torrent pieces through gossiping with neighboring cars. Each car maintains the knowledge of what pieces has fetched through a bitmap. %and, thus, advertise the list of torrent pieces each car has downloaded. DAPES also takes advantage of the bitmap data structure to efficiently encode the state of data fetching. %Instead of having one bit per torrent piece, which may consist of multiple network layer packets, our design directly encodes the state of each network layer data packet in the bitmap.

%CodeTorrent~\cite{lee2006code} makes use of network coding to linearly combine multiple torrent pieces in a single ``coded'' packet, thus, achieving shorter file downloading times in Vehicular Ad-hoc NETworks (VANETs). The authors argue that routing introduces significant overhead for the establishment and maintenance of multi-hop routes due to the wireless medium being error prone, the scale and user density, and the IP address configuration for each node. This argument was verified by our experimental results, showing that DAPES can distribute data resiliently without running a MANET routing protocol due to the data-centric NDN nature.

%BitTorrent for MANETs (BTM)~\cite{rajagopalan2006cross} is another early attempt to apply BitTorrent to MANETs. Peers rely on routing to advertise their torrent pieces, build a list of peers along with the pieces they have and download the desired pieces. As discussed in Section~\ref{ip-experiments}, Bithoc~\cite{krifa2009bithoc, sbai2008bithoc} and Orion~\cite{klemm2003special} are approaches related to our work. DAPES proposes variants of the RPF strategy like Bithoc, however, it does not rely on routing to maintain reachability information to each peer.

%\subsection{Peer-to-Peer Information Data in NDN}

%nTorrent is the closest related work to our design. It is an application to provide P2P file sharing functions natively in NDN, focusing on wired networks~\cite{mastorakis2017ntorrent}. Our design focuses on environments, where intermittent connectivity is the norm. Before the nTorrent proposal, ``FileSync/NDN''~\cite{lindblom2013filesync} implemented a P2P file synchronization in a shared directory among peers over NDN. Detti et al~\cite{detti2013peer, detti2015mobile} and Malabocchia et al~\cite{malabocchia2015using} studied the design of a peer-to-peer video streaming application. Specifically, mobile devices collectively use their mobile connection to download video segments from a server, and share them with each other locally.

%\subsection{Data-centric Disaster Recovery}

%Seedorf et al advocated~\cite{seedorf2015benefit} for the benefits of data-centric name-based communication in disaster recovery scenarios, while different designs to achieve data-centric information dissemination have been proposed~\cite{monticelli2014information, psaras2014name, tagami2016name}. These approaches were mostly based on message flooding or name-based routing. They suggested the use of data carriers to propagate information from one network fragment to others and achieve data replication among distant geographic areas.


